RESAnything: Attribute Prompting for Arbitrary Referring Segmentation

We present an open-vocabulary and zero-shot method for arbitrary referring expression segmentation (RES), targeting input expressions that are more general than what prior works were designed to handle. Specifically, our inputs encompass both object- and part-level labels as well as implicit references pointing to properties or qualities of object/part function, design, style, material, etc. Our model, coined RESAnything, leverages Chain-of-Thoughts (CoT) reasoning, where the key idea is attribute prompting. We generate detailed descriptions of object/part attributes including shape, color, and location for potential segment proposals through systematic prompting of a large language model (LLM), where the proposals are produced by a foundational image segmentation model. Our approach encourages deep reasoning about object or part attributes related to function, style, design, etc., enabling the system to handle implicit queries without any part annotations for training or fine-tuning. As the first zero-shot and LLM-based RES method, RESAnything achieves clearly superior performance among zero-shot methods on traditional RES benchmarks and significantly outperforms existing methods on challenging scenarios involving implicit queries and complex part-level relations. Finally, we contribute a new benchmark dataset to offer ~3K carefully curated RES instances to assess part-level, arbitrary RES solutions.

==> sec/4_method_old.tex <==
\section{Method}
\label{sec:method}

To address the aforementioned challenges of MLLMs requiring large-scale vision-language paired datasets for training, our method introduces a novel approach, which employs systematic attribute prompting of LLMs to generate detailed descriptions of visual properties, enabling rich visual reasoning without extensive annotations.
% ,  to enhance vision-language understanding. 
%We begin by giving an overview of \ourmethod's two-step Chain-of-Thought (CoT) approach for zero-shot visual grounding (Sec~\ref{subsec:method-overview}). We then present the first step, attribute-based prompting pipeline that leverages Large Language Models (LLMs) to analyze target text and image features (Sec~\ref{subsec:attribute-prompting}). Finally, we detail the second step, multi-metric mask proposal selection that converts these attribute-based insights into pixel-level grounding results (Sec~\ref{subsec:grouping-selection}).
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/attribute-prompting.pdf}
    \vspace{-20pt}
    \caption{Attribute prompts generation example of \ourmethod. A reference text $T_r^{ref}$ is generated by instruction from $Q_{ref}$ for description of the target text $T_r$ regarding the image $I$. SAM produces segmentation proposals $M_i$. After post-processing, they are instructed by $Q_{can}$ for LLM to generate candidate texts $T_n^{can}$. } 
    \label{fig:attribute-prompting}
    % \vspace{-10pt}
\end{figure*}

Figure~\ref{fig:overview} provides an overview of \ourmethod{}. Unlike traditional MLLMs that directly connect vision encoders with LLMs, our method consists of two main stages: 1) an attribute prompting stage that leverages SAM and LLM to perform COT reasoning, generating reference text for the target and candidate texts for SAM-generated segmentation proposals (Section~\ref{subsec:attribute-prompting}); 2) a multi-metric mask proposal selection stage that employs LLM as the evaluator to analyze the relationship between candidate and reference texts and produce the final response (Section~\ref{subsec:grouping-selection}).
\label{subsec:method-overview}

\subsection{Attribute Prompting}
\label{subsec:attribute-prompting}
Our first step is generating attribute prompts, both language and visual. %consisting of language prompts and visual prompts. 
Our method employs two types of language prompts: reference text $T_r^{ref}$ and candidate texts $T_n^{can}$.  To enable rich semantic understanding, we design prompts that capture comprehensive object properties and inter-object relationships, going beyond simple object identification.
These language prompts enable us to obtain detailed and relational properties of both the target $T_r$ and proposals. Similar to \cite{sun2024clip}, our visual prompts are a masked image $v_i^m$, and a bounding box image $v_i^b$ corresponding to the segmentation proposal $m_i$ generated from SAM. 

\paragraph{Reference Text Generation.}While most existing referring expressions in current datasets are relatively straightforward, challenging cases like part-level semantic labels and functionality/feature-based descriptions remain difficult for traditional MLLMs. 
These complex queries often provide limited explicit visual information, making accurate localization particularly challenging as MLLMs struggle to directly associate such abstract concepts with image regions. To address this, we generate reference text as a deep reasoning mechanism that bridges abstract descriptions with concrete visual attributes. 
Given an image $I$ and a free-form target text $T_r$, we construct the reference text $T_{ref}^r$ as a single detailed sentence describing the target region by including its description of target attributes $\langle$shape, color, location$\rangle$ in image $I$. Each target corresponds to a unique reference text $T_{ref}^r$. 
The reference text prompt $Q_{ref}$ instructs the LLM to systematically generate the reference text $T_{ref}^r$.
For invisible or irrelevant targets, the reference text provides a reasoned explanation of why the target cannot be localized. 
An example is shown in the top part of the Fig~\ref{fig:attribute-prompting}. Given the target `mesh backrest', the reference text describes its key attributes: `a gray curved mesh backrest with black lining located at the upper portion of the chair'. Details of the reference text prompt $Q_{ref}$ are in supplementary materials.


\paragraph{Segmentation Proposals and Visual Prompts Generation.} Traditional MLLM methods employ end-to-end frameworks with pixel decoders for segmentation, which often generate noisy results when handling complex or abstract queries. To achieve more precise segmentation, we follow CaR~\cite{sun2024clip}'s proposal-based approach but leverage SAM~\cite{kirillov2023segment} instead of CLIP to generate our segmentation proposals. 
While SAM's strong object prior helps produce accurate and coherent region proposals, its raw outputs often include duplicate/overlapping masks and many tiny segments. 
To address these issues, we configure SAM with sampling points at 0.015\% of total image pixels and filter out segments smaller than 0.1\% of the image area, preventing over-segmentation while maintaining meaningful region proposals.
Then we filter duplicate proposals to avoid confusions in following selection. 
Based on the refined segmentation proposals $M_i$, we generate multiple visual prompts $Q_{vis}$ such as bounding box as shown in Fig~\ref{fig:attribute-prompting}. Fig~\ref{fig:visual-prompt} shows different visual prompts. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/visual-prompt.pdf}
    \vspace{-10pt}
    \caption{Example of visual prompts $Q_{vis}$ generated from a segmentation proposal $M_i$.}
    \label{fig:visual-prompt}
    \vspace{-10pt}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/voting.pdf}
    \caption{Illustration of the multi-metric generation step in \ourmethod. Given an input image and target text (e.g., "mesh backrest"), our method first generates a detailed reference text $T_{ref}^r$ via LLM to describe the target's visual attributes. Meanwhile, we produce visual prompts $Q_{vis}$ from the segmentation proposals, each paired with corresponding candidate texts $(T_{can}^i)$ describing their visual characteristics. The reference text bridges abstract functional descriptions with concrete visual attributes, while candidate texts enable comparative analysis. Both text generations are guided by prompts $Q_{C2T}$ and $Q_{R2M}$ separately for comprehensive attribute coverage. The system performs dual-path verification: candidate texts are cross-compared through both LLM reasoning and CLIP text encoders, while segmentation proposals are evaluated via LLM and CLIP image encoders, returning either the most aligned candidate-mask pair or Nil if no suitable match is found.}
    \label{fig:voting}
    % \vspace{-10pt}
\end{figure*}
\paragraph{Candidate Texts Generation.}
We then generate candidate texts $(T_{can}^i)$ that provide detailed descriptions of the segmentation proposals $(M_i)$.
For each segmentation proposal $M_i$, the LLM is instructed by the candidate text prompt $Q_{can}$ and visual prompts $Q_{vis}$ to generate a candidate text $T_{can}^i$, which describes the attributes $\langle$shape, color, location$\rangle$ of the mask region. 
A good visual prompt need to prompt the LLM to focus on the mask region, without removing attribute related information or adding distractions.
Figure~\ref{fig:visual-prompt} shows a few possible representations for visual prompts:
\textit{mask cropped} excels as highlighting the visual attributes, such as shape and color, of the masked region, as the unmasked regions are completely removed, which makes the LLM free from distraction by the irrelevant regions. 
However, it does not provide clear information about the location of the masked region nor its relation with other parts of the image.
In contrast, \textit{bounding box} and \textit{mask contour} provides such relational and locational information, but the bounding box outlines and the mask overlays are distractions when it comes to color and shape.
To alleviate the issues of the respective prompting representations, we concatenate multiple representation in to a single visual prompt $Q_{vis}$, and prompt the LLM to use the most appropriate representation for each type of attribute.
%Therefore, the location attribute and other relation analysis are generated through mask outline or bounding box. 
%Fig~\ref{fig:attribute-prompting} lower part shows an example, where mask images in segmentation proposal share the same color of borders with their corresponding candidate text. 
The complete candidate text prompt $Q_{can}$ is provided in the supplementary materials.

%Similar to reference text $T_{ref}^r$, candidate texts $(T_{can}^i)$ provide detail descriptions of segmentation proposals $(M_i)$. For each segmentation proposal $M_i$, the LLM is instructed by the candidate text prompt $Q_{can}$ and visual prompts $Q_{vis}$ to generate a candidate text $T_{can}^i$, which highlights the attributes $\langle$shape, color, location$\rangle$ of the mask region. As a visual prompt, mask cropped is the best representation of the region in shape and color analysis as its background is pure black, which makes the LLM free from distracting by the irrelevant regions. However, its location and relation regarding the entire image and other regions are unclear. Therefore, the location attribute and other relation analysis are generated through mask outline or bounding box. Fig~\ref{fig:attribute-prompting} lower part shows an example, where mask images in segmentation proposal share the same color of borders with their corresponding candidate text. The complete candidate text prompt $Q_{can}$ is provided in supplementary materials.




\subsection{Multi-metric Mask Proposal Selection}
\label{subsec:grouping-selection}
After obtaining both text and visual prompts from attribute prompting, we employ LLM and CLIP as evaluators to generate assessment metrics for our segmentation proposals $(M_i)$. Fig~\ref{fig:voting} illustrates a detailed example. Each proposal $M_i$ is associated with its candidate text $T_{can}^i$ and visual prompt $Q_{vis}$ (as bounding box, mask crop, or mask overlay). Inspired by ~\cite{sun2024clip}, which uses CLIP to evaluate mask proposals, we leverage both LLM and CLIP to generate comprehensive evaluation metrics. These metrics then serve as inputs to our multi-metric mask proposal selection algorithm to determine the optimal proposal for our target. 

\paragraph{LLM as the Evaluator.}We gather evaluation metrics by comparing the similarity between the target and candidates in text space by comparing the reference text $T_{ref}^r$ with candidate texts $(T_{can}^i)$, which are generated from segmentation proposals. As established in Section~\ref{subsec:attribute-prompting}, each refer has a unique reference text and multiple candidate texts. We use LLM to assess the consistency between each candidate text $T_{can}^i$ and the reference text $T_{ref}^r$ based on described attributes, guided by a comparison prompt $Q_{C2T}$, as shown in lower left of Fig.~\ref{fig:voting}. We constrain the output to binary 'yes'/'no' responses. To address potential instability in these binary responses, we also standardize the LLM outputs. 

Following the text-to-text comparison, we further utilize LLM to evaluate the consistency between the reference text $T_{ref}^r$ and the visual prompts $Q_{vis}$ of segmentation proposals $(M_i)$. This additional evaluation helps mitigate potential errors in candidate text generation, as LLM's performance on visual prompt interpretation may be limited by training data. For each segmentation proposal, we input its visual prompt along with the reference text to LLM, guided by prompt $Q_{R2M}$. Similar to the text comparison, we obtain standardized binary `yes'/`no' responses. 

This dual evaluation strategy ensures more robust matching between the reference text $T_{ref}^r$ and segmentation proposals $(M_i)$, as serve as important inputs for our subsequent selection algorithm, as it considers both textual descriptions and visual representations regarding their attributes.
% This binary comparison focuses specifically on matching attribute descriptions, which we find to be more reliable than attempting to quantify similarities. As a part in our evaluation, LLM excels at understanding and comparing textual descriptions, making them particularly effective at identifying matching attributes between the reference and candidate descriptions. This attribute-focused comparison is crucial for our selection process, as the key to accurate localization lies in finding candidates whose described attributes align closely with those of the target region.

\paragraph{CLIP as the Evaluator.}To gather additional evaluation metrics for our selection algorithm, we employ CLIP to compute similarity scores from both textual and visual perspectives. First, we compute CLIP similarity scores between the reference text $T_{ref}^r$ and candidate texts $(T_{can}^i)$ to assess their semantic alignment in CLIP's embedding space. Subsequently, we calculate CLIP scores between the reference text $T_{ref}^r$ and the mask-cropped visual prompts of segmentation proposals $(M_i)$, providing a complementary vision-language similarity measure. These CLIP-based scores, along with the LLM evaluation results from the previous step, serve as inputs to our final selection algorithm. 

\paragraph{Grouping and Selection.}
Our grouping and selection algorithm prioritizes LLM evaluations while leveraging CLIP scores for fine-grained selection. The algorithm takes as input the reference text $T_{ref}^r$, candidate texts ${T_{can}^i}$, segmentation masks ${M_i}$, LLM binary responses (from both text-to-text ${R_{t2t}^i}$ and text-to-image comparisons ${R_{t2i}^i}$), and CLIP similarity scores ${S_{clip}^i}$. For CLIP scores, we compute \emph{AverageClipScore} as the mean of text-to-text similarity (between $T_{ref}^r$ and $T_{can}^i$) and text-to-image similarity (between $T_{ref}^r$ and mask-cropped image of $M_i$).

\begin{algorithm}
\caption{Grouping and Selection Algorithm}
\label{alg:selection}
\begin{algorithmic}[1]
\Require reference text $T_{ref}^r$, candidate texts $(T_{can}^i)$, segmentation proposals $(M_i)$, LLM text-text responses $(R_{t2t}^i)$, LLM text-image responses $(R_{t2i}^i)$, CLIP scores $(S_{clip}^i)$
\Ensure final segmentation mask $M_i$ or explanation
\State $C_{both} \gets \{M_i | R_{t2t}^i = \text{`yes'} \land R_{t2i}^i = \text{`yes'}\}$
\If{$|C_{both}| = 1$}
    \State \Return single mask $M_i$ in $C_{both}$
\ElsIf{$|C_{both}| > 1$}
    \State $M_{combined} \gets \text{CombineMasks}(C_{both})$
    \State $T_{combined} \gets \text{GenerateCandidateText}(M_{combined})$
    \State $C_{pool} \gets C_{both} \cup \{M_{combined}\}$
    \State \Return $\argmax_{M \in C_{pool}} \text{AverageClipScore}(M)$
\EndIf

\State $C_{t2t} \gets \{M_i | R_{t2t}^i = \text{`yes'}\}$
\If{$|C_{t2t}| = 1$}
    \State \Return single mask in $C_{t2t}$
\ElsIf{$|C_{t2t}| > 1$}
    \State $M_{combined} \gets \text{CombineMasks}(C_{t2t})$
    \State $T_{combined} \gets \text{GenerateCandidateText}(M_{combined})$
    \State $C_{pool} \gets C_{t2t} \cup \{M_{combined}\}$
    \State \Return $\argmax_{M \in C_{pool}} \text{AverageClipScore}(M)$
\EndIf

\State $C_{t2i} \gets \{M_i | R_{t2i}^i = \text{`yes'}\}$
\If{$|C_{t2i}| = 1$}
    \State \Return single mask in $C_{t2i}$
\ElsIf{$|C_{t2i}| > 1$}
    \State $M_{combined} \gets \text{CombineMasks}(C_{t2i})$
    \State $T_{combined} \gets \text{GenerateCandidateText}(M_{combined})$
    \State $C_{pool} \gets C_{t2i} \cup \{M_{combined}\}$
    \State \Return $\argmax_{M \in C_{pool}} \text{AverageClipScore}(M)$
\EndIf

\If{$\max_{i} \text{AverageClipScore}(M_i) < 0.5$}
    \State \Return reference text explanation from $T_{ref}^r$
\EndIf
\State \Return $\argmax_{M_i} \text{AverageClipScore}(M_i)$
\end{algorithmic}
\end{algorithm}
Following a hierarchical selection strategy, the algorithm first identifies candidates with positive responses from both LLM evaluations ($R_{t2t}^i = \text{'yes'} \land R_{t2i}^i = \text{'yes'}$). When multiple candidates satisfy this criterion, we introduce a CombineMasks function that merges these masks through union operations, particularly effective for handling cases where a single semantic entity spans multiple segments (e.g., all legs of a sofa). For the combined mask $M_{combined}$, we generate its candidate text description $T_{combined}$ and include it in the selection pool.

Based on empirical observations that LLM performs more reliably on text-to-text comparisons than text-to-image analysis, we prioritize candidates with positive text-to-text LLM responses ($R_{t2t}^i = \text{'yes'}$) if no candidates satisfy both criteria. The same grouping and selection process applies: combining multiple positive candidates if they exist and selecting based on \emph{AverageClipScore}. If no candidates have positive text-to-text responses, we then consider text-to-image LLM responses ($R_{t2i}^i = \text{'yes'}$) following the same procedure.
As a final verification step, when no candidates receive positive LLM responses, we check if the highest \emph{AverageClipScore} falls below 0.5. This threshold helps identify cases where the target is either invisible or irrelevant to the image, in which case we return the reference text $T_{ref}^r$ explanation that describes why the target cannot be localized. The complete selection process is detailed in Algorithm~\ref{alg:selection}.
